Neural Ray Surfaces for Self-Supervised Learning of Depth and Ego-motion

Self-supervised learning has emerged as a powerful tool for depth and ego-motion estimation, leading to state-of-the-art results on benchmark datasets. However, one significant limitation shared by current methods is the assumption of a known parametric camera model -- usually the standard pinhole geometry -- leading to failure when applied to imaging systems that deviate significantly from this assumption (e.g., catadioptric cameras or underwater imaging). In this work, we show that self-supervision can be used to learn accurate depth and ego-motion estimation without prior knowledge of the camera model. Inspired by the geometric model of Grossberg and Nayar, we introduce Neural Ray Surfaces (NRS), convolutional networks that represent pixel-wise projection rays, approximating a wide range of cameras. NRS are fully differentiable and can be learned end-to-end from unlabeled raw videos. We demonstrate the use of NRS for self-supervised learning of visual odometry and depth estimation from raw videos obtained using a wide variety of camera systems, including pinhole, fisheye, and catadioptric.

==> sections/figure_qualitative.tex <==
%\graphicspath{{figures/}{../figures/}}
\begin{figure*}[ht!]
\centering
\subfloat[Pinhole (KITTI)]{
\includegraphics[width=0.16\textwidth,trim={0 16cm 38cm 0}, clip]{figures/experiments/kitti_0000000042.png}
\includegraphics[width=0.16\textwidth,trim={0 16cm 38cm 0}, clip]{figures/experiments/kitti_0000000124.png}
\includegraphics[width=0.16\textwidth,trim={0 16cm 38cm 0}, clip]{figures/experiments/kitti_0000000522.png}
\includegraphics[width=0.16\textwidth,trim={0 16cm 38cm 0}, clip]{figures/experiments/kitti_0000001259.png}
\includegraphics[width=0.16\textwidth,trim={0 16cm 38cm 0}, clip]{figures/experiments/kitti_0000001653.png}}
\begin{comment}
\\
\vspace{-2mm}
\subfloat[Pinhole (Multi-FOV) \vitor{TODO}]{
\includegraphics[width=0.16\textwidth,trim={0 0cm 38cm 0}, clip]{figures/experiments/fov_fisheye_0000000005.png}
\includegraphics[width=0.16\textwidth,trim={0 0cm 38cm 0}, clip]{figures/experiments/fov_fisheye_0000000277.png}
\includegraphics[width=0.16\textwidth,trim={0 0cm 38cm 0}, clip]{figures/experiments/fov_fisheye_0000000885.png}
\includegraphics[width=0.16\textwidth,trim={0 0cm 38cm 0}, clip]{figures/experiments/fov_fisheye_0000001536.png}
\includegraphics[width=0.16\textwidth,trim={0 0cm 38cm 0}, clip]{figures/experiments/fov_fisheye_0000001965.png}}
\end{comment}
\\
\vspace{-2mm}
\subfloat[Fisheye (Multi-FOV)]{
\includegraphics[width=0.16\textwidth,trim={0 0cm 38cm 0}, clip]{figures/experiments/fov_fisheye_0000000005.png}
\includegraphics[width=0.16\textwidth,trim={0 0cm 38cm 0}, clip]{figures/experiments/fov_fisheye_0000000277.png}
\includegraphics[width=0.16\textwidth,trim={0 0cm 38cm 0}, clip]{figures/experiments/fov_fisheye_0000000885.png}
\includegraphics[width=0.16\textwidth,trim={0 0cm 38cm 0}, clip]{figures/experiments/fov_fisheye_0000001536.png}
\includegraphics[width=0.16\textwidth,trim={0 0cm 38cm 0}, clip]{figures/experiments/fov_fisheye_0000001965.png}}
\\
\vspace{-2mm}
\subfloat[Catadioptric (OmniCam)]{
\includegraphics[width=0.16\textwidth,height=5.5cm,trim={0 0cm 29cm 0}, clip]{figures/experiments/omnicam_0000011810.png}
\includegraphics[width=0.16\textwidth,height=5.5cm,trim={0 0cm 29cm 0}, clip]{figures/experiments/omnicam_0000010698.png}
\includegraphics[width=0.16\textwidth,height=5.5cm,trim={0 0cm 29cm 0}, clip]{figures/experiments/omnicam_0000001826.png}
\includegraphics[width=0.16\textwidth,height=5.5cm,trim={0 0cm 29cm 0}, clip]{figures/experiments/omnicam_0000000536.png}
\includegraphics[width=0.16\textwidth,height=5.5cm,trim={0 0cm 29cm 0}, clip]{figures/experiments/omnicam_0000000086.png}}
\\
% \vspace{-2mm}
\caption{\textbf{Qualitative depth estimation results for different camera geometries} using our proposed NRS framework. Note that all these results were obtained using the same architecture and parameters (Figure \ref{fig:diagram}); the only modification are the video sequences used for training and inference.
}
\label{fig:qualitative}
\end{figure*}


==> supp_sections/figure_diagram.tex <==


\begin{figure}[ht!]
\centering
\includegraphics[width=0.9\textwidth]{figures/theory/diagram3.pdf}
\caption{\textbf{Proposed self-supervised monocular depth, pose and ray surface estimation framework}. Both depth and ray surface decoders share the same encoder backbone, and by combining the predicted depth map $\hat{D}_t$ with the predicted ray surface $\hat{\mathbf{Q}}_t$, we are able to perform the view synthesis necessary for self-supervised learning.}
\label{fig:diagram}
\end{figure}
\vspace{-3mm}
